Harvesting Brownian Motion: Zero Energy Computational Sampling

The key factor currently limiting the advancement of computational power of electronic computation is no longer the manufacturing density and speed of components, but rather their high energy consumption. While it has been widely argued that reversible computation can escape the fundamental Landauer limit of $k_B T\ln(2)$ Joules per irreversible computational step, there is disagreement around whether indefinitely reusable computation can be achieved without energy dissipation. Here we focus on the relatively simpler context of sampling problems, which take no input, so avoids modeling the energy costs of the observer perturbing the machine to change its input. Given an algorithm $A$ for generating samples from a distribution, we desire a device that can perpetually generate samples from that distribution driven entirely by Brownian motion. We show that such a device can efficiently execute algorithm $A$ in the sense that we must wait only $O(\text{time}(A)^2)$ between samples. We consider two output models: Las Vegas, which samples from the exact probability distribution every $4$ tries in expectation, and Monte Carlo, in which every try succeeds but the distribution is only approximated. We base our model on continuous-time random walks over the state space graph of a general computational machine, with a space-bounded Turing machine as one instantiation. The problem of sampling a computationally complex probability distribution with no energy dissipation informs our understanding of the energy requirements of computation, and may lead to more energy efficient randomized algorithms.

==> fragments.tex <==
\subparagraph*{Molecular computing}
Since the earliest work proposing reversible computing as a way to minimize energy consumption, molecular computation has been evoked as a powerful thought experiment~\cite{bennett1973logical,bennett1982}.
Bennett recognized that enzymes modifying an information-carrying polymer---similar to those prevalent in biology---could perform arbitrary information processing,
and that logically reversible computation could be embedded in a physically reversible manner and driven forward with arbitrarily little energy per step of computation.

While Bennett's proposed enzyme lacked mechanistic details, advances in DNA nanotechnology provide a potential way to engineer such computation using DNA strand displacement cascades~\cite{qian2011efficient,thachuk2012space,yahiro2016implementation}.
Experimentally, DNA-based reversible logic circuits have been realized~\cite{genot2011reversible,orbach2012logic}.
Using DNA strand displacement reactions localized on a surface is a particularly promising direction for experimental implementations of reversible molecular computation~\cite{brailovskaya2019reversible}.

$$\ldots$$

Note that biochemical stochasticity has an essential role in key cellular activities~\cite{eldar2010functional}, 
so designing biochemical systems that can sample from nontrivial distributions may be useful for engineering desirable cell behavior.

\subparagraph*{Entropy and energy}
While general physical systems can be modeled with high complexity and with many alternative frameworks for their dynamics, we choose to focus purely on a thermodynamic model of energy and entropy. In particular, we employ a model in which a (closed) system can be decomposed into a set of micro-states, which are the finest-grained distinguishable physical configurations of the entire system. All micro-states of the system are assumed to have the same total energy. The set of micro-states is then partitioned into macro-states, also called logical states, and the number of micro-states subsumed by a given logical state represents the \emph{entropy} of that logical state. More concretely, if $W_a$ is the set of micro-states which all correspond to logical state $a$, then $a$ has entropy $k\ln|W_a|$, where $k$ is Boltzmann's constant. 

We tend to think of a state transition as thermodynamically favorable if the final state has more entropy than the initial state, and vice versa.  More formally, we let $G$ be the system's Gibbs free energy, and say that $\Delta G=-T\Delta S$ for a given state transition with entropy change $\Delta S$. Operations with negative values of $\Delta G$ represent releases of energy, and are thermodynamically favorable, so we expect them to occur more readily than operations whose $\Delta G$ is higher. 


When focusing on the particular energetic and entropic mechanisms of a \emph{computational} system, we base our work on the fundamental observations of Landauer \cite{Lan61}. In particular, we take the principle that each logically irreversible operation carried out on a bit of information reduces the entropy of a computational system by $k\ln2$. A logically irreversible operation entails setting a logical bit to zero or one independently of its initial configuration, which we otherwise call ``erasing'' a bit of information. Recalling our definition of entropy, this quantity $k\ln 2$ can now be derived from the fact that erasing a bit of information halves the number of micro-states present in the current logical state. Each such operation therefore must, to conserve the total thermodynamic entropy of the enclosing system, release a minimum of $kT\ln2$ Joules of energy into the surroundings, where $T$ is the temperature. We will refer to this minimum as the \emph{Landauer limit}. As such, it is typically the case that a computational machine will release an amount of heat which grows asymptotically with the length of its computational task---unless, of course, the machine or task is designed specifically as a composition of logically reversible operations. The latter choice is the fundamental principle guiding the design of both our Las Vegas and Monte Carlo computational sampling constructions, allowing them to run at effectively a zero-energy cost.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subparagraph*{Physical Embedding of a Machine.}
In order to connect our computational model with our energy models, we present the notion of a physical embedding of a machine.
Any physical realization of a machine will necessarily map logical configurations to physical configurations, each with potentially different amounts of stored energy $\Delta G$.
%In reality, each of these configurations (macro-states) is comprised of some number of other physical configurations (micro-states) and Brownian motion essentially executes a random walk over these configurations.\todo{AL: add details for heat release, Landaur's, and number of micro-states?}
To account for this behavior, we consider the realization of a general machine as a continuous-time Markov process that we call a physical embedding.


% [version that directly uses Metropilis dynamics]
% \begin{definition}
%     Let $M = (\Sigma, f)$ be a general machine.
%     A \emph{physical embedding} of $M$ is an undirected graph $P_M = (V, E)$ with vertices $V = \Sigma$ and edges $E = \{(U,W) \mid W \in f(U)\}$ (i.e., $(U,W) \in E$ if $W$ is a successor configuration of $U$). 
%     Each vertex $U$ is assigned a value $\Delta G_U \in \mathbb{R}$, and each edge $(U,W)$ is assigned a weight dictated by Metropolis dynamics\footnote{Note that any other reasonable kinetic model can be used.}.
% \end{definition}

\begin{definition}
    Let $M = (\Sigma, f)$ be a general machine.
    A \emph{physical embedding} of $M$ is a directed graph $P_M = (V, E)$ with vertices $V = \Sigma$ and edges $E = \{(U,W) \mid W \in f(U) \text{ or } U \in f(W) \}$ (i.e., if $W$ is a successor configuration of $U$ then they are connected by forward and backward edges). 
    Each vertex $U$ is assigned a value $\Delta G_U \in \mathbb{R}$, and each edge $(U,W)$ is assigned the weight $\lambda_{U \to W}$ dictated by Metropolis dynamics~(\Cref{eqn:metropolis}).
\end{definition}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subparagraph*{Thermodynamics / Kinetics and Computation.} 
\todo{DS: I am tempted to cut this section}
%Any physical implementation of a general machine is a physical system and is therefore subject to this equilibrium constraint. 
\todo{AL: want to rework this paragraph to motivate zero energy computation---maybe re-emphasize that we're focused on equilibrium thermodynamics}
If we consider a physical embedding of a general machine to be a closed system with fixed volume and temperature, then the system's probability distribution at equilibrium is the Boltzmann distribution.
One may be tempted to design output configurations to have a lower $\Delta G$ (making them more favorable), in order to bias the distribution at equilibrium towards these configurations.
However this comes with two major problems.
First, to reset the machine energy must be expended to return it to the initial configuration.
Second, execution of the machine may release heat which must either be extracted from the system via an energy-expensive cooling mechanism or will decrease the effectiveness of the energy barrier in future executions of the machine.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\todo{DS: remove this paragraph since we no longer use ``computation graph''?}
A general machine $(\Sigma, f)$ can also be thought of in terms of a graph with vertex set $\Sigma$ and edges defined using $f$:
\begin{definition}
    Let $M = (\Sigma, f)$ be a general machine.
    Then its \emph{computation graph} $G_M = (V,E)$ is the  directed graph with vertices $V=\Sigma$ and edges $E=\{(U,W) \mid W \in f(U)\}$.
    In other words, there is a edge from $U$ to $W$ whenever $W$ is a possible successor configuration of $U$.
\end{definition}
Our notion of a deterministic machine $M$ directly corresponds to all vertices of $G_M$ having out-degree at most one, and for a reversible machine $M$ all vertices additionally have in-degree at most one.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






For our Monte Carlo construction we design a zero energy distribution sampler such that if the observer waits sufficiently long between measurements, they will always yield samples from a distribution with negligible distance from independent samples of the target distribution.
%The observer will only ever need to read the output register, so it will not need to expend any energy to forget metadata.
As before we will start with the simpler case where the desired distribution is uniform over $r$ bits.
\paragraph*{Sampling the uniform distribution}
Our Monte Carlo Construction works by ``linking'' two otherwise independent copies of a machine so that a step ``forward'' in one machine causes the other machine to step ``backwards.''
To formalize this, we need to define the notion of a layered general machine.

\begin{definition}
A general machine $M= (\Sigma, f)$ is \emph{$T$-layered} if there is a partition of $\Sigma$ into layers $L_1, \ldots, L_T$ such that for all $\sigma \in L_i$, $f(\sigma) \subseteq L_{i+1}$.
\end{definition}

Intuitively a $T$-layered machine always runs in $T$ steps and during step $i$, the machine will be at state in $L_i$.
Given $T$-layered machines $M_1 = (\Sigma_1, f_1)$ and $M_2 = (\Sigma_2, f_2)$, we can couple them to get a single machine that performs both computations while still being $T$-layered.
If $M_1$ has layers $L_1^1, \ldots, L_T^1$ and $M_2$ has layers $L_1^2, \ldots, L_T^2$ then the coupled machine $M$ has state space $\Sigma = (L_1^1 \times L_1^2) \cup \ldots \cup (L_T^1 \times L_T^2)$.
The action of $M$ is defined using the function $f(\sigma_1, \sigma_2) = (f_1(\sigma_1),f_2(\sigma_2))$.
Note that as long as $\sigma_1 \in L_i^1$ and $\sigma_2 \in L_i^2$ then this value will be in layer $i+1$ of $\Sigma$ and our new machine is also $T$-layered.

Coupling two machines as described above can be extremely useful when considering zero energy computation.
Specifically, two independent machines will take independent random walks over their state space.
However, if the two sub-machines are coupled then the coupled machine will always be in a configuration where both sub-machines have a state in the same layer.
This key observation lets us build a zero energy Monte-Carlo distribution sampler.

To sample from the uniform distribution over $r$ bits, we will start with a machine $M$ composed of a randomizer over $r$ bits as described in the Las Vegas construction.
On each node in the final column of the randomizer, we append a chain of length $r+1$ containing the appropriate bitstring as output.\footnote{As with the Las Vegas machine, we can have the randomizer keep the current bitstring both in the work and output registers so that the machine is only making local changes during each step.}
We observe that this computation graph can be directly interpreted as a layered machine with $2r+2$ layers where the $r+1$ columns of the randomizer make up layers $L_1, \ldots, L_{r+1}$ and the chains make up layers $L_{r+2}, \ldots L_{2r+2}$.

Let $M^{-1}$ be the machine described above except with the order of the layers reversed.
We will construct coupled machine $M^*$ by coupling $M$ and $M^{-1}$.
Note that since $M^{-1}$ contains a sample from the uniform distribution in layers $L_1, \ldots L_{r+1}$ and $M$ contains a sample in layers $L_{r+2}, \ldots L_{2r+2}$, one of the two machines will have a sample whenever $M^*$ is measured.
Thus we can add a meta-data value to the states of $M^*$ that is set to $-1$ when the machine is in layers $L_1, \ldots L_{r+1}$ and set to $1$ when the machine is in layers $L_{r+2}, \ldots, L_{2r+2}$.
By first reading the meta-data, an observer can then know which sub-machine's output should be read to give the current output value.

Let $c>0$ be a constant. The observer of this machine acts as follows: They wait time $c\cdot r^2$ before measuring the meta-data of the machine's state. If they observe a $-1$ or a $1$ they then read the part of the output register corresponding to sub-machine $M^{-1}$ or $M$ respectively and record what they observe as output.
This process is repeated each time the observer wants to collect a sample.

\begin{lemma}
After time $c r^2$, the probability that observing the state of the machine does not yield an independent uniformly random sample is exponentially small in $c$.
\end{lemma}
\begin{proof}
Proof sketch: there *should be* a constant probability of hitting the end of the line (which resets the randomness) from any starting state in time that is $O(r^2)$. We can thus break time into chunks of length $O(r^2)$ and for each chunk the machine should have an (independent) $O(1)$ probability of hitting the end. We can then use a Chernoff bound to give us an exponential tail.
\end{proof}
\paragraph*{Extending to arbitrary distribution sampling}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Version II}
\todo{NK: this is kind of informal right now. We should more clearly define what our configurations look like.}
We start with a simplified version of our construction for sampling $r$ uniform random bits and then extend it to sample from any distribution where there is an algorithm that maps $r$ uniformly random bits to an element of that distribution.
Our construction will have the property that its configurations contain a single piece of metadata set to one of three configurations.
Reading this metadata and comparing its value to that of the last successful sample is sufficient to determine if the machine has produced a new independent sample from the distribution.

The construction will guarantee that after sufficient time, the value of this metadata will indicate that a new independent sample can be taken with probability at least $1/4$.
Therefore after $t$ sufficiently spaced reads of the machine, it will have produced a new sample from the distribution with probability at least $1-(3/4)^t$.
We note that the number of required samples for any success probability $p$ is independent both of the desired number of random bits $r$ needed to seed the sampling algorithm and the length of the algorithm's computation.

\paragraph*{Sampling the uniform distribution}
We start with a zero energy machine that samples from the uniform distribution over $r$ bits with the above guarantees regarding the metadata at thermodynamic equilibrium.
Our machine contains a "randomizer" composed of $(r+2)2^{r+1}$ configurations arranged into $r+2$ columns that each have $2^{r+1}$ nodes.
For each column $i\in \{0,\ldots, r+1\}$ and bitstring $b$ of length $r+1$, one node represents the configuration $((b,i), 0, \emptyset)$.
We then add edges between configurations $((b,i), 0, \emptyset)$ and $((b',i'), 0, \emptyset)$ when $i = i'+1$ and $b=b'$ or $b$ and $b'$ only differ on the $i$'th coordinate.

\begin{lemma}
crossing the randomizer randomizes the value of $b$ in the work space \todo{find a formal way to state this}
\end{lemma}
\begin{proof}
\end{proof}

As we just showed, a random walk that starts on one end of the graph and ends on the other will end in a configuration with a uniformly random bitstring.
Thus we can use metadata to indicate if we are on the left or right side of the randomizer and we know that after this metadata changes, our samples are independent of one another.

We now add to the construction so that we can "store" the first $r$ bits of the random bistrings created by being at a state on either side of the randomizer.
We will introduce $(r+2)2^{r+2}$ additional nodes that will be used to store outputs.
Each of these nodes is assigned a configuration $((b,i), \text{sign}(i), b_r)$ for all $b \in \{0,1\}^{r+1}$ and $i \in \{-(r+2), \ldots -1, 1, \ldots, (r+2)\}$.
There are edges between these new nodes where their values of $i$ differs by $1$ and their values of $b$ only differ on the last bit.
There are edges between the node in the randomizer with configuration $((b,0), 0, \emptyset)$ and the new pair of nodes with configurations $((b',-1), -1, b'_r)$ where $b_r = b'_r$.
Likewise there are edges between the nodes in the randomizer with configuration $((b,r+1),0,\emptyset)$ and the new pair of nodes with configurations $((b',1),1,b'_r)$ where $b_r = b'_r$.

This is possible by adding a chain of length $r+1$ to all nodes on the leftmost and rightmost sides of the randomizer.
Let $b_r$ be the first $r$ bits of $b$.



Specifically, for each bitstring $b$ we add a chain of $r+2$ nodes with configurations $((b,i),-1, b_r)$ to each node with configuration $((b,0), 0, \emptyset)$ and a chain of $r+2$ nodes with configurations $((b,i),1,b)$ to each node with configuration $((b,r),0,\emptyset)$.\footnote{If you want the machine to only change a constant number of bits per step, you can design the randomizer so that it keeps the respective value of $b$ in the output register as it changes its value in the work register.} An example of this construction when $r=2$ is shown in \cref{fig:LV-simple}.

\begin{figure}
    \centering
    \includesvg[width=.6\textwidth]{images/LV-simple.svg}
    \caption{Our Las-Vegas construction to sample uniformly random bitstrings of length 2. The circle nodes are the randomizer and have metadata value zero. The square nodes on the left and the right are the output holding regions and have metadata values $-1$ and $1$ respectively. For simplicity, we show only the bistring associated with each node instead of the full configuration.}
    \label{fig:LV-simple}
\end{figure}

Now our computation is divided into three parts: two output holding regions assigned with meta data values $-1$ and $1$ and a randomizer region assigned meta data $0$.
An observer can collect independent samples from the machine with the following strategy:
The first time the observer measures the metadata register and finds a value $m$ such that $|m| = 1$, the observer measures the output register $o$ and then records the pair $(m_1,o_1) = (m,o)$.
For the $i$'th sample, the observer periodically measures the metadata register until they find the value $m$ such that $|m_{i-1} + m| = 0$. They then measure output register $o$ and record the pair $(m_i, o_i) = (m,o)$.

At thermodynamic equilibrium there will be a $1/3$ chance of observing the necessary metadata to record a new sample. However, if we only want a $1/4$ chance of this, then we can get away without waiting for thermodynamic equilibrium.
\begin{lemma}\label{lem:lv-sample-time}
    After time ?\todo{NK: I think this will be $O(r^2)$ but we should prove this.}, sampling the metadata of the above machine gives at least a $1/4$ probability of observing the necessary value to make a new independent sample.
\end{lemma}
\begin{proof}
    
\end{proof}
Thus we have designed an abstract machine that can generate independent samples of $r$ uniformly random bits while only requiring a constant number of observations per sample.

\paragraph*{Extending to arbitrary distribution sampling}\todo{we probably want to have quotable theorem statements and embed most of the following in a proof block.}
The above construction can be extended to sample from any distribution where a deterministic machine can map $r$ uniformly random bits to a sample from that distribution.
We will assume that $M$ is some general machine that completes this task starting at the configuration $(b,0,\emptyset)$.
Without loss of generality, $M$ can be constructed so that the metadata register always has the value $0$.
Also, we can use the reversible pebble game to modify $M$ so that it is a reversible machine.
We will then assume that $T$ -- the (maximum) time complexity of $M$ on any input -- is known to our construction.
We will again modify $M$ so that it takes time $T$ on any input.
This can be achieved by augmenting the work register for the configurations of $M$ with a timer that counts down from $T$ to $0$.
We will further elongate the computation of $M$ by having the counter continue from $0$ to $-(2T+r)$.
We will have two copies of this machine: $M_{-1}$ and $M_{1}$ and then change the metadata on the respective machines in the sates where the counter has negative values to $-1$ or $1$ respectively.
In the states where the counter has a non-negative value, we instead add $-1$ or $1$ to the work register.
We then couple the randomizer as described in the simple case to $M_{-1}$ on the left and $M_{1}$ on the right.
We do this by adding an edge from each node with configuration $((b,0),0,\emptyset)$ in the randomizer to $((b,-1),0,\emptyset)$ in $M_{-1}$.
Likewise we add an edge from each node $((b,r),0,\emptyset)$ in the randomizer to $((b,1),0,\emptyset)$ in $M_{1}$. This construction can be seen in \cref{fig:LV-general} \todo{try to make it more clear what we are doing.}

\begin{figure}[t]
    \centering
    \includesvg[width=.9\textwidth]{images/LV-general.svg}
    \caption{The general Las-Vegas construction. $R$ is the randomizer while $M_1$ and $M_{-1}$ are two copies of a general machine that computes samples from the desired distribution. The grey regions indicate that the metadata is set to either $1$ or $-1$ and this state of the machine contains a sample.}
    \label{fig:LV-general}
\end{figure}

Similar to the construction for uniformly random bits, the metadata partitions the states into three groups: two that have outputs on opposite sides of the construction and one that indicates that computation is still in process.
We will use the same general procedure for generating samples to guarantee their independence.
By using the timer to extend the region with determined outputs, we again have a $1/3$ probability at thermodynamic equilibirum of being at an output containing state on a specific side of the graph.
Thus by the same reasoning as in \cref{lem:lv-sample-time}, if we wait at least ? time between samples, there will be a $1/4$ chance that the observed metadata implies that we can get an independent sample from the distribution.




%%%%%%%%%%%%%%%%%%%%%%%%%%



\paragraph*{Time, space, and energy}
There is a long history of work regarding saving space at the cost of additional time.
With limited memory, values often must be recomputed, which increases the time of a computation when we decrease its space.
These trade-offs were first studied in restricted models of computation represented using pebble games, where pebbles are placed onto and removed from a graph in correspondence to how an algorithm chooses to compute and forget fixed intermediate values during its computation \cite{Tom80, BFK+81, Ben89, AB16}.
Tight time-space tradeoffs have also been established for more general models of computation by bounding the amount of progress that can be made in a small number of steps and a bounded amount of initial state \cite{BC82, Abr91, BSSV03, KSdW07, BK23}.

In general, additional space can be used in lieu of energy to bias computation in the forward direction.
As pointed out in \cite{Lan61, Ben03}\todo{NK: check that these are the right source for this} heat must be released to bias computation towards the deletion of bits; however, this idea can be flipped on its head.
By replacing bits with fixed values with random assignments, we can use entropy to drive our computation in the desired direction.
Additionally constructions like \cite{Ben89} use auxiliary space to make computation reversible, which allows it to be completed with only a small overhead in time and arbitrarily little energy per step.

It is no secret that using additional energy can cause computation to go faster.
On standard hardware, concepts like overclocking allow faster computation at the cost of additional energy \cite{}.
For quantum computation, the adiabatic method can be compressed to arbitrarily small time scales at the cost of a blow up in energy \cite{}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now define what we mean by a sampling problem.


\begin{definition}\todo{make part of the main text instead of formal def}
    Let $\calA$ be some procedure that produces elements from some distribution $\calD$. Then $\calA$ \emph{$\varepsilon$-samples} any distribution $\calD'$ where $\norm{\calD - \calD'} \leq \varepsilon$. We say that $\calA$ \emph{exactly-samples} distribution $\calD'$ when $\calD = \calD'$.
\end{definition}
%We now introduce two complementary approaches to solving sampling problems: Monte Carlo and Las Vegas, in the sense of \cite{Els80}.
Now we can give precise definitions to our Monte Carlo and Las Vegas machines.
\begin{definition}
    A machine $M = (\Sigma, f)$ \emph{Monte Carlo} samples a distribution $\calD$ with time $T$ and accuracy $\varepsilon$ if after starting in some state $I\in\Sigma$ and running for some time $T$, the distribution of configurations of $M$ is $\varepsilon$-close to $\calD$.

    A zero energy distibution sampling machine $M = (\Sigma, f)$ \emph{Las Vegas} samples a distribution $\calD$ with expected time $T/p$ if ... \todo{NK: I am not sure exactly how to define this without making the state space more specific. Ie. we need an indicator saying when a sample is good to read. More generally we need to discuss how to convert elements of $\Sigma$ to samples} 
\end{definition}
%\begin{definition}
%    A general machine $M$ and observer $O$ execute a \emph{Monte Carlo} algorithm for sampling problem $\mathcal{D}$ if:
%    \begin{enumerate}
%        \item $M$ solves $\mathcal{D}$ approximately
%        \item Each time that $O$ observes $M$'s c, she can extract and record an answer corresponding to a draw from the approximate distribution $\mathcal{D}'$
%    \end{enumerate}
%\end{definition}
%\begin{definition}
 %   A general machine $M$ and observer $O$ execute a \emph{Las Vegas} algorithm for sampling problem $\mathcal{D}$ if:
 %   \begin{enumerate}
 %       \item $M$ solves $\mathcal{D}$ exactly
 %       \item When $O$ observes $M$'s c, she will with some constant probability accept this configuration (i.e. $M$ is in a halt c) and record a draw from $\mathcal{D}$. If she rejects the c, no answer is recorded and $M$ is allowed to continue running until the next observation.
 %   \end{enumerate}
%\end{definition}
%We will give two generic minimal auxiliary energy constructions in this paper: one (Las Vegas) that exactly samples from a valuable distribution $\mu$ using a constant expected auxiliary energy cost and another (Monte Carlo) that can approximate $\mu$ with zero auxiliary energy cost. 
\subsection{Useful gadgets} There are a couple of design motifs for low energy computation that fit naturally into our constructions in this paper. We expect that these tricks will also be useful in the construction of other low energy machines.

\paragraph*{Reversible Computation} The reversible pebble game \cite{Ben89} is a powerful tool that lets us take any deterministic computation graph and convert it into a set of disjoint chains (which are reversible) where the source nodes represent inputs and the reachable sink node contains the corresponding output.
This process comes with a small overhead in the time (length of the chains) and space (number of configurations) complexities.

When trying to execute deterministic irreversible computation on a zero energy machine, our kinetic model will cause irreversible steps to occur in the backwards directions more frequently than in the forwards direction.
This can lead to an exponential number of steps in the time of the algorithm before reaching the end of the computation.
After turning the state space into a collection of chains, the kinetic behavior of a zero energy machine looks like an unbiased one dimensional walk which will reach the end of the computation in time that is at most the square of the length of the chain.\todo{with high probability?}
\todo{add stuff here about why our computation graph being a chain is optimal if we care about resetting it}

\paragraph*{Output Holding Regions} It is a desirable property that after letting a zero energy machine run for sufficient time, measuring the machine is likely to give the desired output.
While most traditional algorithms halt after producing their output, implementing this behavior on a zero energy machine that has $n$ reachable configurations where only one of them contains the output would give us only a $1/n$ probability of measuring that output at thermodynamic equilibrium.
This probability can be artificially amplified by adding redundant configurations to the machine after it has produced its output.
One simple way to do this is by generating $r$ random bits after producing the output.
However, this approach results in an "entropy trap" that takes expected time that is exponentially large in $r$ for the machine to escape if resetting the machine is desirable.

If we have already made the algorithm reversible, we can simply add a counter that counts up during the computation's execution and after finding the output, counts back down to zero.
Doing so guarantees that at thermodynamic equilibrium there is always a $1/2$ probability of measuring the output.
Additionally this technique avoids the entropy trap described above and therefore is useful when resetting the machine is a desirable property.

\paragraph*{Batteries and Energy Coupling} If there are entropically favorable steps in a computation graph (like generating random bits) that you want to make unbiased, then these steps can be coupled with entropically unfavorable steps in an auxiliary computation so that the net behavior is entropy neutral. 
This is especially desirable when we want a random walk to quickly traverse over these steps in either direction.
A simple example of this is when a computation generates $r$ uniformly random bits, we can couple it with a process that erases $r$ random bits.
That way the entropy remains constant regardless of where you are in this process allowing us to convert a computation that is heavily forward-biased into a uniform random walk.

==> reversible-counter.tex <==
\section{Reversible Turing Machine Counter}\label{sec:rev-counter}
Here is our construction for a reversible Turing machine counter.
The machine acts on a tape that starts with $\log_2 T$ zeroes with the head on the right and will increment the value on the tape $T = 2^k$ times before halting.
The machine enters the state $\beta$ on a blank tape before each time it tries to increment the counter and enters state $\xi$ while the tape is blank after it has finished incriminating the counter.
By changing the transition rules for entering and leaving these states, the counter can be used to count the number of steps made by another Turing machine.
This counter runs in $O(T)$ steps and its implementation is fully reversible.
The Turing machine counts with the least significant bit on the right and the machine halts when it has counted to $T$
Here are its transition rules:
\begin{align*}
    \beta &\to (\alpha, L)\\
    (\alpha, 1) &\to (\beta, 0)\\
    (\alpha, 0) &\to (\gamma, 1)\\
    (\xi, 0) &\to (\gamma, 0)\\
    (\xi,\_) &\to (\beta, \_)\\
    \gamma &\to (\xi, R)
\end{align*}
The machine is reversible since no two transition rules give the same configuration.
The machine runs in time linear in $T$ by an amortized argument regarding how far the head needs to move to the left for each step.\todo{formalize this argument}
